Accelerating Bandwidth-Bound Deep Learning Inference with Main-Memory Accelerators

DL inference queries play an important role in diverse internet services and a large fraction of datacenter cycles are spent on processing DL inference queries. Specifically, the matrix-matrix multiplication (GEMM) operations of fully-connected MLP layers dominate many inference tasks. We find that the GEMM operations for datacenter DL inference tasks are memory bandwidth bound, contrary to common assumptions: (1) strict query latency constraints force small-batch operation, which limits reuse and increases bandwidth demands; and (2) large and colocated models require reading the large weight matrices from main memory, again requiring high bandwidth without offering reuse opportunities. We demonstrate the large potential of accelerating these small-batch GEMMs with processing in the main CPU memory. We develop a novel GEMM execution flow and corresponding memory-side address-generation logic that exploits GEMM locality and enables long-running PIM kernels despite the complex address-mapping functions employed by the CPU that would otherwise destroy locality. Our evaluation of StepStone variants at the channel, device, and within-device PIM levels, along with optimizations that balance parallelism benefits with data-distribution overheads demonstrate $12\times$ better minimum latency than a CPU and $2.8\times$ greater throughput for strict query latency constraints. End-to-end performance analysis of recent recommendation and language models shows that StepStone PIM outperforms a fast CPU (by up to $16\times$) and prior main-memory acceleration approaches (by up to $2.4\times$ compared to the best prior approach).

==> Makefile <==
PAPER = main
TEX = $(wildcard *.tex)
BIB = $(wildcard bib/*.bib)
FIGS = $(wildcard fig/*.pdf fig/*.png graphs/*.pdf graphs/*.png)
VIEW = open 

all: clean $(PAPER).pdf view

.PHONY: all clean

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) Makefile
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex --synctex=-1 $(PAPER)
	sed -i  -e 's/\/cygdrive\/c/C:/g' $(PAPER).synctex


view:
	$(VIEW) $(PAPER).pdf

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf



==> tex/gemm_pim_old.tex <==
\section{StepStone PIM}
\label{sec:gemm}

In this section, we present \textit{StepStone PIM} that enables independent GEMM execution with PIMs under any XOR-based memory-system address mapping. In StepStone PIM, the weight matrix is partitioned and assigned to PIMs based on underlying address mapping and each PIM works on the assigned part of the GEMM in a collaborative manner. In the CPU's point of view, it looks as if PIMs are jumping around and stepping only the stones (i.e. cache blocks) that are physically local to them.
\mattan{Maybe be explicit about targeting the numerous relatively small, high aspect-ratio matrices found in many ML-inference tasks?}

\subsection{Overview}
\label{subsec:gemm_overview}

\fig{fig:overview}{b} shows three matrices that are involved in our target GEMM operation. Main assumption is that the large matrix A (i.e. the weight matrix in FC layers) resides in DRAM while the small input matrix B (i.e. input activation) can be either in the CPU cache or DRAM. Before GEMM, matrix B should be replicated to the private memory region of each PIM (mechanisms for allocating private memory region is explained in Section \ref{subsec:mech_malloc}). Portion of the matrix B that are used by each PIM depends on address mapping, matrix size and aspect ratio, and the DRAM hierarchy level in which PIM is conducted. In our example, all 4 PIMs need the entire matrix B, which is the worst case in terms of replication overhead. After the replication, all the input operands reside in the local memory of PIMs so that they can concurrently execute GEMM. During GEMM execution, cache blocks of matrix B are copied from DRAM to the scratchpad memory and reused multiple times while cache blocks of matrix A is read once and discarded after being used. Matrix C (i.e. output pre-activation) will be also buffered in the scratchpad memory and drained later. Once partial GEMM is complete in all the PIMs, partial matrix Cs should be reduced into one matrix to get the final result. Given this execution flow, to benefit from PIM, the replication and reduction overheads should be amortized over numerous PIM computations. In addition, to minimize the data movement between the scratchpad memory and DRAM, PIMs should reuse buffered data in the scratchpad memory as much as possible. 
%
%The rest of this section is focused on enabling the GEMM execution described above and, specifically, solving the following questions.
%
%\begin{itemize}
%	\item What should be considered to allocate memory for PIM?
%	\item How can PIMs maximally reuse their scratchpad memory (a.k.a PIM buffer)?
%	\item How can PIMs maximally exploit row-buffer locality?
%	\item How can PIMs identify the next cache block to process while considering both of these row-buffer and PIM-buffer localities? 
%\end{itemize}

\begin{figure*}[t!]
\centering
        \includegraphics[width=0.8\textwidth]{fig/overview.pdf}
	\caption{Overview of GEMM execution with StepStone PIM.}
	\label{fig:overview}
\end{figure*}


%\subsection{Memory Allocation for Private/Shared Memory Regions}
%\label{subsec:gemm_malloc}
%Two memory regions are accessed by PIMs during PIM acceleration: shared and private regions. Both regions can be accessed by the CPU but they have different access interface (see Section \ref{subsec:mech_access_pvt_mem} for details). Data in the shared region can be accessed normally by the CPU and are distributed across multiple PIMs such as matrix A in \fig{fig:overview}.b. If the shared region spans more PIMs, we can achieve higher parallelism during the actual GEMM execution. However, spanning more PIMs is not always beneficial since matrix B should be replicated to and matrix C should be reduced among more PIMs, which may incur high overhead. Therefore, memory allocator should consider this trade-off, assign appropriate number of PIMs for GEMM, and take that into account when allocating frames for PIM execution. Once the number of PIMs is determined, memory allocator should allocate frames such that the frames span the target number of PIMs and are well-distributed across those PIMs to balance loads. 
%
%The PIM-aware memory allocation is also required when allocating memory space for private memory regions. The private regions are used to store matrix B and partial results of matrix C of each PIM. Therefore, to allocate private memory space, the frame IDs should be selected such that those frames reside in the target PIMs. With the Skylake address mapping, one 4-KB frame spans 4 banks (2 channels ${\times}$ 2 banks from different bank groups). Considering different PIM levels, this corresponds to 4, 2, and 2 PIMs for bank group-, rank-, and channel-level PIMs. Therefore, to efficiently use memory space, the PIMs that share the same frame should execute together (such as PIM 0, 1, 8, and 9 in our example). 
%
%Another important factor that affects PIM performance is row-buffer locality (RBL). Unlike the CPU, PIMs have limited bank-level parallelism, thereby exploiting RBL directly impacts memory performance. To maximally exploit RBL, all the cache blocks in an opened DRAM row should be consumed before switching to the different one of the same bank. This can be done by allocating memory in a coarse granularity. With the Skylake address mapping, a 4-KB page only occupies one eighth of each row in 4 different banks. On the other hand, contiguous 8 frames span entire rows of those 4 banks, thereby the minimum allocation granularity should be 32 KB to maximize RBL.

\subsection{Exploiting Temporal Locality with StepStone Block Grouping}
\label{subsec:gemm_grouping}

%\fig{fig:overview}.b illustrates which parts of the large input matrix (i.e. matrix A) are assigned to each PIM as a results of our baseline address mapping (\fig{fig:overview}.a). Each small blocks in matrix A represents a cache block and its label represents the index of the PIM that is in charge of processing it. We assume that the matrix is stored in a row-major order. The most straight-forward way to process these cache blocks is to access them in the ascending physical-address order. However, if the other matrices (i.e. matrix B and C) do not fit in the PIM buffer, data should move between DRAM and the PIM buffer. In such case, maximally reusing the PIM buffer is the key to achieve high PIM performance. To maximize PIM buffer reuse, we propose \textit{sub-matrix grouping}. Once the groups are formed, PIMs execute GEMM for one group at a time. This group-wise execution is basically processing all the cache blocks in the matrix A that need currently buffered data to do GEMM. 

\fig{fig:overview}{b} illustrates which parts of the large input matrix (i.e. matrix A) are assigned to each PIM as a results of our baseline address mapping (\fig{fig:overview}{a}). Each small blocks in matrix A represents a cache block and its label represents the ID of the PIM that is in charge of processing it. We assume that the matrix is stored in a row-major order. The cache blocks with same color share the same parts of matrix B and C as input and output operands, respectively. Therefore, to maximally exploit temporal locality captured by the scratchpad memory, we need to execute GEMM operations for the same-color blocks first and move onto the blocks with different colors. We call this method of grouping cache blocks based on data sharing pattern as \textit{StepStone block grouping}. 

To generally apply this StepStone block grouping to any XOR-based address mapping, we need to understand what determines the number of groups and how to identify the cache blocks that belong to same group. In our example, we assume PIMs are assigned for each bank group. Therefore, to identify which PIM has certain cache block in its local memory, the physical address of the cache block is converted into DRAM address with CPU's address mapping and PIM ID is obtained by concatenating the channel (1 bit), rank (1 bit), and bank group IDs (2 bits) (\fig{fig:overview}{a} (above)). In this case, we say that there are four PIM ID bits. Given this information, the number of groups is determined by ${2^x}$, where ${x}$ is the number of PIM ID bits that are partly determined by lower ${\log_{2}K + 2 (= k)}$ bits and partly by ${(k, k + \log_{2}M]}$ bits of the physical address, where ${K, M}$ are the number of columns and rows of matrix A, respectively (+2 for 4-byte elements). We call the former bit field as \textit{MCOL} field and the latter as \textit{MROW} field since they determine the matrix column and row indices, respectively. In our example, there are two PIM ID bits (CH and BG0 bits) that satisfies this condition. Therefore, there are ${2^2 (= 4)}$ groups per PIM as we can confirm from the figure. 

The question is why does this condition determines the number of groups. The intuition behind the answer is as follows: If the PIM IDs are calculated partly by MROW and partly by MCOL fields, matrix-row indices determine the PIM interleaving pattern within each matrix row. The rows with the same interleaving pattern can form a StepStone block group. Specifically, the interleaving pattern is determined by the XOR results in the MROW field that partly determine CH (i.e. \texttt{b19} ${\oplus}$ \texttt{b18} ${\oplus}$ \texttt{b13} ${\oplus}$ \texttt{b12}) and BG0 IDs (i.e. \texttt{b14}). Concatenation of these two intermediate XOR results becomes a group ID. The matrix rows with different group IDs have different PIM interleaving pattern since the bits in matrix column indices are XOR-ed with group IDs and finally determine the PIM ID for each cache block. StepStone block grouping works for any address mapping as long as the matrix A is aligned in a 2D space where the number of matrix columns is a power of 2 when elements are stored in a row-major order and the number of matrix rows is a power of 2 when stored in a column-major order. 

\subsection{StepStone Address Generation}
\label{subsec:gemm_addr_gen}
To enable group-wise GEMM after forming StepStone block groups, each PIM should find the cache blocks that belong to a specific group. We call this behavior of finding the next cache block to process as \textit{StepStone address generation}. The generated physical address will be converted to DRAM address within PIMs and checked if the address belongs to the target group of the target PIM. The simplest method is to increment physical address by one cache block and check if that cache block belongs to the target group of current PIM. Otherwise, PIMs just keep incrementing the physical address until they find the match. We call this method as \textit{increment-and-check}. This method may work if there are only few PIMs in the system. However, as the number of PIMs increases, performance scalability will be limited by the incrementing overhead. In addition, for some address mappings with coarse-grained address interleaving, only a fraction of PIMs will be active while the others remain idle by just incrementing to find the next cache block.

To mitigate the incrementing overhead, we propose a new mechanism called \textit{increment-correct-and-check}. The correction step is the key to reduce the amount of meaningless incrementation and it is composed of three parts: instant and iterative corrections, and carry forwarding. \fig{fig:overview}{c} (above) shows an example of these correction mechanisms when current PIM ID and target group IDs are both 0 and the physical address is incremented from 0x40 to 0x80. Since the current PIM ID is 0, all the channel, rank, BG1, and BG0 IDs should be 0 for the target cache blocks. However, since \texttt{b7} of the physical address 0x80 is set, BG0 ID becomes 1. This means that PIM 0 should find the next physical address that has the \texttt{b7} value 0. The instant correction logic sets \texttt{b7} to 0 and generate a carry to \texttt{b8}. If the correction happens for 0 ${\rightarrow}$ 1, carry will not be generated. Note that if a carry is generated, the StepStone address generator will not check the corrected physical address. 

In the next iteration, \texttt{b8} will be incremented by 1 (carry) and CH ID becomes 1. Therefore, another instant correction is required to set \texttt{[b9, b8]} from 01 to 11. This is because the outcome of \texttt{Goup ID[0] ${\oplus}$ b9 ${\oplus}$ b8} should equal to current \texttt{PIM ID[0]}, 0. In this way, if contiguous bits are used to determine the same PIM ID bit, they can be corrected together and save one or more iterations. We call this routine of iteratively adding carry and applying the instant correction as \textit{iterative correction}. 

% Carry forwarding
We can further save the number of iterations by using \textit{carry forwarding}. The effect of carry forwarding is to skip a large chunk of address regions that do not have cache blocks that belongs to current PIM. This can be applied to some bits that are used to determine group (e.g. \texttt{b14}) and PIM IDs (e.g. \texttt{b16 and b15}). In the Skylake address mapping, \texttt{b14} corresponds to \texttt{Group ID[3]} and this should be fixed to certain value depending on the group currently being processed. On the other hand, \texttt{b16} and \texttt{b15} are used to determine \texttt{PIM ID[1]} and \texttt{PIM ID[2]}, respectively. For PIM 0, the bit pairs \texttt{[b20, b16]} and \texttt{[b19, b15]} can only be either 00 or 11. Therefore, as long as \texttt{b20} and \texttt{b19} do not change, \texttt{b16} and \texttt{b15} should be fixed to either 0 or 1 during address incrementation. As a result, the carry from \texttt{b13} can be directly forwarded to \texttt{b17} during the correction step and jump over the large memory regions that do not have any cache blocks for PIM 0.

% Tiling
The same carry forwarding mechanism can be used for partitioning group matrices. We refer to the one large logical matrix that are formed by block grouping as \textit{group matrix}. If a group matrix is relatively large so that corresponding parts of matrix B and C do not fit in the PIM buffer, it should be partitioned into smaller sub-matrices. Since the elements are stored in row-major order, partitioning in vertical direction means that a part of matrix rows should be skipped while generating addresses. This can be done by applying the carry forwarding to the most-significant bits in the MCOL field. Note that the number of partitions also should be a power of 2. 

%\subsection{Restricting Grouping to Maximize Row-Buffer Hits}
%\label{subsec:gemm_max_rb_hits}
%% 512KB granularity
%Optimizing only for PIM buffer reuse can sometimes significantly degrade PIM performance due to low DRAM row-buffer hit rate. In each DRAM row, cache blocks from different groups are colocated. If the size of group matrix is large, it will span multiple DRAM rows per bank. Then, the naive group-wise GEMM execution will incur low row-buffer hits since only a small fraction of DRAM rows will be accessed and switched to the next DRAM rows. To solve this problem, we introduce a horizontal grouping boundary for matrix A. That is, even though group IDs are the same, sub-matrices cannot be grouped across this boundary. All the groups within the boundary will be first executed and then move onto the next horizontal partition and repeat this process. This grouping restriction improves row-buffer locality at the cost of PIM buffer reuse.



%\subsection{Capacity Optimization with Matrix Bonding}
%\label{subsec:gemm_bonding}
%% Low row-buffer hit ratio due to the power-of-2 constraint
%As stated in Section \ref{subsec:gemm_grouping}, matrix A should be aligned in the 2D space with power-of-2 matrix columns. If the number of matrix columns is not a power-of-2, we allocate a bigger memory space of which size is the smallest power-of-2 columns that is greater than ${K}$. Then, PIMs only use ${K}$ matrix columns. The unused matrix columns can be skipped using similar mechanism to StepStone address generation. For instance, the smallest GPT-2/3 model includes MLP layers where ${K}$ equals to 768 and 3072, respectively. In both cases, a quarter of matrix space in unused. To solve this problem, we bond multiple narrower row-major matrices and form a larger matrix of which size is equivalent to that of matrix A. That is, when ${K}$ is 768, we create three matrices with 256 matrix columns and logically bond them by grouping sub-matrices across the matrix boundaries. Even for the matrix with power-of-2 ${K}$, matrix bonding can be beneficial. \fig{fig:matrix_bonding} shows an example of bonding two matrices which are equivalent to the matrix A (\fig{fig:overview}.b). With matrix bonding, there are only 2 groups as opposed to 4 groups as in the original matrix A. This means that the total data that should be moved from DRAM to the scratchpad memory becomes half. The impact of the number of StepStone block groups is shown in Section \ref{subsec:buffer_size}. Note that the number of groups is decreased only because \texttt{b14} has been excluded from the MROW field as a result of halving the matrix size. Consequently, only PIM ID[0] is determined by both MROW and MCOL fields.
%
%\begin{figure}[t!]
%\centering
%        \includegraphics[width=0.38\textwidth]{fig/matrix_bonding.pdf}
%	\caption{Matrix bonding.}
%	\label{fig:matrix_bonding}
%\end{figure}




\subsection{Performance Optimization for Small Weight Matrix}
\label{subsec:opt_tradeoff}
When the matrix size is relatively small, replication and reduction overhead dominates the overall execution time. In such case, we can use a subset of PIMs as opposed to activating all of them. Instead, we loose performance for GEMM operation but this tradeoff can be beneficial when the overheads are dominant. We show this tradeoff in Section \ref{subsec:eval_tradeoff}. Another optimization for relatively small matrix A is that CPU can directly write to and read from PIM's scratchpad memory when the matrix B and C fits in it. This reduces the time to move data between DRAM and the scratchpad memory. 


%Three registers are required  for the StepStone address generator to track the current physical address of all three matrices. Whenever the physical address crosses 256-element boundary (i.e. 16 cache blocks), the current-address register should be switched to the next one in a round-robin manner. 

%One potential problem is that if the sub-matrices of the same group across matrices happen to be located in the different DRAM rows of the same bank, the number of row-buffer hits will significantly decrease. Therefore, we need to ensure that they are always located in different banks. Moreover, to group across matrix boundary, matrices should be properly aligned in the physical address space. These should be considered at memory allocation time. The detailed mechanisms and memory allocation considerations are explained in Section \ref{subsec:mech_matrix_bonding} and Section \ref{subsec:mech_malloc}, respectively.

%\subsection{Discussion: Enabling Multiple Processing Options with One Data Instance}
%With the StepStone address generation mechanism, we can enable different levels of PIMs to execute GEMM without data reorganization. That is, only one instance of matrix A is needed in the system and either the CPU or PIMs in the different memory hierarchy levels can access it as is. This feature of StepStone PIM gives great flexibility when deciding the right place to execute for different situations and matrix shapes. For instance, if majority of matrix-A elements are stored in the CPU caches, we can assign the GEMM workload to the CPU; otherwise, we assign it to PIMs. Switching execution between the CPU and PIM is light-weight since the large data is already shared and both can access them in high speed. Also, since PIMs in different memory hierarchy levels have different advantages, we can leverage them based on resource requirements. Lower-level PIMs, such as bank group-level PIMs, have higher peak memory bandwidth and efficiency whereas have high area/power constraints so that the performance of their processing elements will be low. On the other hand, higher-level PIMs have relatively lower peak memory bandwidth whereas have higher area/power budgets to integrate high-performance vector units. In this way, our StepStone PIM can provide efficiency and flexibility to the system, which are the key requirements in data-center computing. We explore this trade-offs in Section ?.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tex/implementation_old.tex <==
\section{Detailed Mechanisms}
\label{sec:impl}

In this section, we explain the detailed mechanisms of StepStone PIM. Without loss of generality, we assume that the Skylake address mapping, bank group-level PIM, 4-KB frame are used when explaining the mechanisms unless stated otherwise. 

\subsection{Baseline PIM System}
\label{subsec:baseline_system}
Figure \ref{fig:baseline_system} illustrates the baseline architecture of our PIM system. The host-side PIM controller interfaces between the CPU and PIMs and is mainly in charge of initiating and completing the PIM kernel launched by the CPU. We consider three-levels of PIM designs: (1) channel-, (2) device-, and (3) bank group-(BG)level PIM. Though the channel- and rank-level PIMs can operate independently to other PIMs in the same level, BG-level PIMs are not entirely independent due to rank-level timing parameters, such as tRCD and tFAW. These timing parameters affect row operations to different bank groups such that ACT commands should be sequentialized within a rank and issued back-to-back by keeping time intervals defined by those timing parameters. Therefore, we put an extra PIM control logic at the I/O port of each chip to deal with this row operations. Whenever an ACT command should be issued to open a row, the BG-level PIMs should first query the control logic to determine when to issue the command. 

Each PIM can be controlled and monitored through the memory-mapped control/status registers. The sizes of scratchpad memory and SIMD units depend on the area budget. Based on our area estimate, StepStone-BGs have 8-width SIMD units and 8-KB scratchpad memory, which takes 0.15 ${mm}^2$ of area, and StepStone-DVs have 32-width SIMD units and 32-KB scratchpad memory per PIM, which takes 1.2 ${mm}^2$ of area. These areas are comparable to prior bank-level \cite{gu2020ipim} and device-level PIM designs \cite{asghari2016chameleon}. Note that these are areas and performance per DRAM device so we need to multiply by the number of chips to get the aggregated scratchpad memory size and peak PIM performance. We assume that the aggregated scratchpad memory size and peak PIM performance of StepStone-DV is equivalent to one StepStone-CH. The pipeline depth of PIM should be deep enough to tolerate the minimum DRAM latency defined by tCL; otherwise, PIMs cannot fully utilize the DRAM bandwidth. 

\begin{figure*}[t!]
\centering
        \includegraphics[width=0.85\textwidth]{fig/baseline_system.pdf}
	\caption{The architecture of baseline PIM system.}
	\label{fig:baseline_system}
\end{figure*}

\subsection{PIM-aware Frame Allocation}
\label{subsec:mech_malloc}

As explained in Section \ref{subsec:gemm_overview}, there are private and shared memory regions that PIMs access during execution. Though the data-layout requirements are different between those two regions (described in \ref{subsec:mech_access_pvt_mem}), the requirements for memory allocation is the same: the regions should span the target PIMs. As explained in Section \ref{subsec:opt_tradeoff}, we sometimes use only a subset of PIMs due to the performance tradeoffs in StepStone PIM. Based on the decision of target number of PIMs, we allocate physical frames such that they span only the target number of PIMs. For instance, the minimum PIM granularity for StepStone-BG is 4 when the Skylake address mapping is used, since that is the number of bank groups that one frame spans. We refer to these 4 PIMs as a \textit{PIM group}.

Once the number of PIM groups to activate is determined, say 2, we allocate memory for private and shared regions as follows. First, we set the minimum allocation granularity to 32KB, which corresponds to 8 contiguous frames that share the same rows of the same banks. To make sure that the allocated space spans two different PIM groups, it is required to specify PIM group ID when allocating frames. The PIM group ID bits correspond to bit 15 and 16 in our case since they determine other PIM ID bits than the ones that are determined by the frame offset field (\fig{fig:overview}.a). Therefore, we adopt the PIM-aware frame coloring mechanism, similar to the ones introduced by Chopim \cite{cho2020near}. This can be done by maintaining dedicated free lists of frames for each PIM group. That is, we use at least two colors to color bit 15 and 16 when allocating frames in 32-KB granularity. Also, we can easily integrate this 32-KB frame coloring in modern memory allocators, such as tcmalloc \cite{ghemawat2009tcmalloc} and jemalloc \cite{evans2011scalable}. These allocators have multiple free lists of pages based on the contiguous memory chunk size. We break the free list for 32-KB memory chunk into 4 based on the PIM group ID. Then, when a special memory allocation API is called with a target PIM group ID, the memory allocator just need to choose frames from the corresponding free list. The private region can be allocated using the same interface. For the 2-MB huge page, one page already spans all the banks in the system, so it is impossible to choose the target PIM counts in the same way as the 4-KB frame case. Instead, we choose different PIM levels to balance the trade-off between parallelism and replication/reduction overhead.


\subsection{Accessing Private Memory Region from the CPU}
\label{subsec:mech_access_pvt_mem}

The CPU accesses the private memory region of PIM for two reasons: to replicate input matrix and to reduce the partial results. During replication, we reorganize the input matrix for each PIM such that PIMs can access it in order during its group-based execution. \fig{fig:replication} illustrates the reorganization process. The outer-most loop is for the weight-matrix columns in a cache-block granularity. With the column ID and address mapping, we can identify the PIM and group IDs of all the cache blocks in the weight matrix that will be dot-producted with corresponding input-matrix column. This can be done efficiently by fixing the MCOL field to current column ID (\fig{fig:overview}.a) and consider all possible outcomes for group IDs. Then, the PIM and group ID pair can be generated. For each PIM-group pair, we copy one cache block at a time (e.g. \texttt{a0}). Then, in the inner-most loop, we iterate over other cache blocks of the input-matrix column (e.g. \texttt{a1}, \texttt{a2}, and \texttt{a3}). As a result, the table in the right will be generated. Since we know the base address of the private memory region and destination PIM and group ID, the destination physical address can be generated using the StepStone address generation mechanism. The reduction process can be done in a similar manner such as group-wise reduction across the PIMs that process the same matrix rows.

\begin{figure}[t!]
\centering
        \includegraphics[width=0.48\textwidth]{fig/replication.pdf}
	\caption{Input-matrix Reorganization.}
	\label{fig:replication}
\end{figure}


\subsection{Partitioning within StepStone Block Group}
\label{subsec:mech_part}
If operands of one StepStone block group do not fit in the scratchpad memory, group matrix should be partitioned into smaller blocks. As explained in Section \ref{subsec:gemm_addr_gen}, partitioning in vertical direction can be done with carry forwarding when generating addresses for the weight matrix. For horizontal partitioning, matrix rows should be partitioned into multiple-of-16 rows for single-precision elements. We assume that the output matrix is stored in a column-major order and this restriction enables to align results within the cache block. 

\begin{algorithm}[h]
\SetAlgoLined
 // hrz\_parts: Horizontal partitions\;
 // ss\_groups: StepStone block groups\;
 // vrt\_parts: Vertical partitions\;
 \For{hpart in hrz\_parts}{
  buffer\_fill(C)\;
  \For{grp in ss\_groups}{
  	\For{vpart in vrt\_parts}{
  	  buffer\_fill(B)\;
  	  StepStone GEMM\;
  	}
  }
  buffer\_drain(C)\;
 }
 \caption{Group-based GEMM with partitioning}
\end{algorithm}

\subsection{Execution Flow of StepStone GEMM}
\label{subsec:mech_pim_flow}
% What information does the CPU provide to each PIM?
% Vector unit
As a result of input-matrix reorganization (Section \ref{subsec:mech_access_pvt_mem}), the input matrix is aligned in the private memory region such that operands for each group matrix are stored contiguously. Therefore, PIMs can stream the data from DRAM to the scratchpad memory when loading the input matrix parts that correspond to the operands for current group. After the input matrix blocks are loaded to the scratchpad memory, the PIM control logic generates the next physical address (using StepStone address generation) to read from DRAM and convert it into DRAM address. To do this, the PIM controller in the CPU side should provide the base physical address of the weight matrix. Once the cache block of weight arrives in the DRAM operand buffer (\fig{fig:baseline_system}), it will be dot-producted with all the cache blocks of input matrix across batch dimension. That is, if the batch size is 4, one cache block will be dot-producted with 4 different cache blocks in the scratchpad memory. To keep up the data transfer rate of DRAM, the SIMD unit should have corresponding computation throughput. Therefore, the requirement for SIMD unit width will increase along with the batch size. The partial output matrix will be accumulated within each PIM and will later be reorganized during the reduction step to get the final output. 

%
%\subsection{Enabling Matrix Bonding}
%\label{subsec:mech_matrix_bonding}
%% TODO: probably might have to discuss the impact of matrix bonding on CPU execution
%Matrix bonding requires to group sub-matrices across the matrix boundaries. To enable this, all the matrices involved in the matrix bonding should be first aligned such that the starting group ID is the same. For instance, if the first matrix row of one matrix corresponds to group ID 0, this should also be the case for other matrices that are bonding targets. Then, to apply the StepStone address generation to the bonded matrix, multiple registers are required to track the progress on each matrix. Let us assume that three matrices with 256 matrix columns are well aligned (as mentioned above) and bonded together. In such case, three registers are required for the StepStone address generator to track the current physical address of all three matrices. Whenever the physical address crosses 256-element boundary (i.e. 16 cache blocks), the current-address register will be switched to the next one in a round-robin manner. Note that the behavior of switching registers is equivalent to crossing the matrix boundary. 




